Enhancing Text-to-SQL Translation for Financial System Design

Text-to-SQL, the task of translating natural language questions into SQL queries, is part of various business processes. Its automation, which is an emerging challenge, will empower software practitioners to seamlessly interact with relational databases using natural language, thereby bridging the gap between business needs and software capabilities. In this paper, we consider Large Language Models (LLMs), which have achieved state of the art for various NLP tasks. Specifically, we benchmark Text-to-SQL performance, the evaluation methodologies, as well as input optimization (e.g., prompting). In light of the empirical observations that we have made, we propose two novel metrics that were designed to adequately measure the similarity between SQL queries. Overall, we share with the community various findings, notably on how to select the right LLM on Text-to-SQL tasks. We further demonstrate that a tree-based edit distance constitutes a reliable metric for assessing the similarity between generated SQL queries and the oracle for benchmarking Text2SQL approaches. This metric is important as it relieves researchers from the need to perform computationally expensive experiments such as executing generated queries as done in prior works. Our work implements financial domain use cases and, therefore contributes to the advancement of Text2SQL systems and their practical adoption in this domain.

==> figures/Parameters.tex <==
\def\range{8}
\def\xyRatio{3/4}
\def\circSize{1mm}

\begin{tikzpicture}[->, very thick, align=center, scale=0.8]
  
  \draw (0,-0.5) -- (0,\range*\xyRatio) node[below right, draw=none] {Parameters};
  \draw (-0.5,0) -- (\range,0) node[above, draw=none] {Year};
  \foreach \n\t in {1/2018,2/2019,3/2020,4/2021,5/2022,6/2023}
  \node[below,draw=none] at (\n*1.2,0) {$\t$};
  \foreach \n\t in {1/8,2/9,3/10,4/11,5/12}
  \node[left,draw=none] at (0,\n) {$10^{\t}$};
  \draw[dashed, gray, shorten <=5] (0,0) -- (\range,\range*\xyRatio);

  \foreach \n/\name/\abbr in {1.5/BERT(340M)/, 3/GPT-2(1.5B)/HF, 4/T5(11B)/MP2, 6.5/PaLM(540B)/CISD, 7.3/GPT-4(1.7T)/CCSD(T)}
  \fill[blue!60!black] (\n,\xyRatio*\n) circle (\circSize) node[right=1ex, black, draw=none] (\abbr) {\name};

%   \draw[red, thick] (HF) -- (SE);
  \fill[blue!60!black] (6,4.5*\xyRatio) circle (\circSize) node[right=1ex, black, draw=none] {GPT-NeoX(20B)};
  \fill[blue!60!black] (7,5.2*\xyRatio) circle (\circSize) node[right=1ex, black, draw=none] {LLaMA(70B)};

  \fill[blue!60!black] (4.1,6*\xyRatio) circle (\circSize) node[left=1ex, black, draw=none] {GPT-3(175B)};
\end{tikzpicture}


==> figures/Transfomers.tex <==

\begin{forest} 
for tree={
    edge path={
      \noexpand\path[\forestoption{edge}](!u.parent anchor) -- +(5pt,0) |- (.child anchor)\forestoption{edge label};},
    grow=0,
    reversed, % tree direction
    parent anchor=east,
    child anchor=west, % edge anchors
    anchor=west,
    if n children=0{tier=word}{}
}
[Transformer\cite{vaswani2017attention}
[BERT\cite{devlin2018bert}
[T5\cite{raffel2020exploring}
[Flan-T5\cite{chung2022scaling}[PaLM\cite{anil2023palm}]]
] ]
[GPT-Neo-X\cite{black2022gptneox}[CodeGen\cite{nijkamp2022codegen}[nsql\cite{numbersstation2023NSText2SQL}][CodeGen2\cite{nijkamp2023codegen2}]][Pythia\cite{biderman2023pythia}][StarCoder\cite{li2023starcoder}]]
[LLaMA\cite{touvron2023llama}
 [ALPACA\cite{alpaca}] [Koala\cite{koala_blogpost_2023}] [MPT\cite{MosaicML2023Introducing}] 
[LLaMA-2\cite{touvron2023llama2}] ] 
[GPT\cite{radford2018improving}
[GPT-2\cite{radford2019language}[GPT-3\cite{brown2020language}[GPT-4\cite{openai2023gpt4}]]] ] ] 
\end{forest}







==> sections/RQs/RQ1.tex <==

\sectopic{RQ1. } \textit{Which solution alternative is the most accurate for Text2SQL converstion?}
%

==> sections/RQs/RQ2.tex <==

\sectopic{RQ2. } \textit{What is the effect of the proposed techniques and postprocessing steps on the performance of the alternative solutions?}



==> sections/RQs/RQ3.tex <==

\sectopic{RQ3. } \textit{Which solution alternative is the most efficient in terms of execution time and computational resources?}


==> sections/RQs/RQ4.tex <==
\sectopic{RQ4. } Will these new metrics evaluate SQL queries and Ground Truth as accurately as Execution Match when the original database is unreachable?


==> sections/RQs/RQ5.tex <==
\sectopic{RQ5. } Text-to-SQL tasks in financial scenarios (especially banks) are lacking in existing datasets. How should we solve it?

==> tables_results/BLEU.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\begin{tabular}{llr}
\hline
Model Type                         & Model Name               & \multicolumn{1}{l}{All} \\ \hline
\multirow{8}{*}{General LLM}       & ChatGPT-3.5-turbo        & 33.6                    \\
                                   & Davinci                  & 34.9                    \\
                                   & MPT-7B-instruct          & 19.3                    \\
                                   & ALPACA-7B                & 20.5                    \\
                                   & KOALA-7B                 & 10.9                    \\
                                   & OpenAssistant-pythia-12B & 16.0                    \\
                                   & Falcon-7B-instruct       & 7.9                     \\
                                   &                          & \multicolumn{1}{l}{}    \\ \hline
\multirow{4}{*}{Code Specific LLM} & CodeGen2-7B              & 26.4                    \\
                                   & Starcoder-15.5B          & 28.7                    \\
                                   & Vicuna-7B                & 12.2                    \\
                                   & nsql-6B                  & 44.3                    \\ \hline
\multirow{2}{*}{Seq-to-Seq Model}  & T5-3B(tscholak/cxmefzzi) & 24.3                    \\
                                   & PICARD+T5/3B             & 24.9                    \\ \hline
\end{tabular}
\end{table}

==> tables_results/Error.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{llrrrrr}
\hline
Model Type                         & Model Name               & \multicolumn{1}{l}{no such table} & \multicolumn{1}{l}{syntax error} & \multicolumn{1}{l}{incomplete input} & \multicolumn{1}{l}{no such column} & \multicolumn{1}{l}{All} \\ \hline
\multirow{8}{*}{General LLM}       & ChatGPT-3.5-turbo        & 0                                 & 79                               & 1                                    & 22                                 & 0.082                   \\
                                   & Davinci                  & 78                                & 25                               & 0                                    & 31                                 & 0.236                   \\
                                   & MPT-7B-instruct          & 141                               & 36                               & 33                                   & 276                                & 0.020                   \\
                                   & ALPACA-7B                & 21                                & 13                               & 4                                    & 360                                & 0.031                   \\
                                   & KOALA-7B                 & 36                                & 175                              & 31                                   & 393                                & 0.002                   \\
                                   & OpenAssistant-pythia-12B & 91                                & 45                               & 2                                    & 387                                & 0.025                   \\
                                   & Falcon-7B-instruct       & 240                               & 98                               & 91                                   & 310                                & 0.002                   \\
                                   &                          & \multicolumn{1}{l}{}              & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}                 & \multicolumn{1}{l}{}               & \multicolumn{1}{l}{}    \\ \hline
\multirow{4}{*}{Code Specific LLM} & CodeGen2-7B              & 4                                 & 58                               & 116                                  & 168                                & 0.124                   \\
                                   & Starcoder-15.5B          & 1                                 & 20                               & 44                                   & 148                                & 0.059                   \\
                                   & Vicuna-7B                & 4                                 & 661                              & 0                                    & 35                                 & 0.002                   \\
                                   & nsql-6B                  & 10                                & 1                                & 8                                    & 235                                & 0.032                   \\ \hline
\multirow{2}{*}{Seq-to-Seq Model}  & T5-3B(tscholak/cxmefzzi) & 9                                 & 16                               & 1                                    & 104                                & 0.409                   \\
                                   & PICARD+T5/3B             & 0                                 & 72                               & 16                                   & 2                                  & 0.371                   \\ \hline
\end{tabular}
\end{table}

==> tables_results/Exact_Match.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{llrrrrr}
\hline
Model Type                         & Model Name               & \multicolumn{1}{l}{Level 1} & \multicolumn{1}{l}{Level 2} & \multicolumn{1}{l}{Level 3} & \multicolumn{1}{l}{Level 4} & \multicolumn{1}{l}{All} \\ \hline
\multirow{8}{*}{General LLM}       & ChatGPT-3.5-turbo        & 0.184                       & 0.146                       & 0.008                       & 0.000                       & 0.082                   \\
                                   & Davinci                  & 0.434                       & 0.469                       & 0.133                       & 0.000                       & 0.236                   \\
                                   & MPT-7B-instruct          & 0.015                       & 0.054                       & 0.033                       & 0.000                       & 0.020                   \\
                                   & ALPACA-7B                & 0.037                       & 0.092                       & 0.000                       & 0.000                       & 0.031                   \\
                                   & KOALA-7B                 & 0.000                       & 0.008                       & 0.000                       & 0.000                       & 0.002                   \\
                                   & OpenAssistant-pythia-12B & 0.041                       & 0.063                       & 0.000                       & 0.000                       & 0.025                   \\
                                   & Falcon-7B-instruct       & 0.007                       & 0.000                       & 0.000                       & 0.000                       & 0.002                   \\
                                   &                          & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}    \\ \hline
\multirow{4}{*}{Code Specific LLM} & CodeGen2-7B              & 0.199                       & 0.293                       & 0.042                       & 0.000                       & 0.124                   \\
                                   & Starcoder-15.5B          & 0.116                       & 0.113                       & 0.025                       & 0.000                       & 0.059                   \\
                                   & Vicuna-7B                & 0.000                       & 0.008                       & 0.000                       & 0.000                       & 0.002                   \\
                                   & nsql-6B                  & 0.045                       & 0.071                       & 0.033                       & 0.000                       & 0.032                   \\ \hline
\multirow{2}{*}{Seq-to-Seq Model}  & T5-3B(tscholak/cxmefzzi) & 0.610                       & 0.573                       & 0.592                       & 0.127                       & 0.409                   \\
                                   & PICARD+T5/3B             & 0.513                       & 0.556                       & 0.492                       & 0.135                       & 0.371                   \\ \hline
\end{tabular}
\end{table*}

==> tables_results/Executable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}




==> tables_results/Model_list.tex <==
\begin{table*}[]
\begin{tabular}{lrrrrr}
\hline
Model Name               & \multicolumn{1}{l}{Model Size} & \multicolumn{1}{l}{Input Style} & \multicolumn{1}{l}{Code Dataset} & \multicolumn{1}{l}{Fine-Tuned} & \multicolumn{1}{l}{Pure-Code Output} \\ \hline
ChatGPT-3.5-turbo        &                                & Prompt                          &                                  &                                & Nearly Yes                           \\
Davinci                  &                                & Instruct                        &                                  &                                & Yes                                  \\
MPT-7B-instruct          & 7B                             & Instruct                        &                                  &                                & No                                   \\
ALPACA-7B                & 7B                             & Prompt                          &                                  &                                & No                                   \\
KOALA-7B                 & 7B                             & Prompt                          &                                  &                                & No                                   \\
OpenAssistant-pythia-12B & 12B                            & Prompt                          &                                  &                                & No                                   \\
Falcon-7B-instruct       & 7B                             & Prompt                          &                                  &                                & No                                   \\
                         & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{}            & \multicolumn{1}{l}{}             & \multicolumn{1}{l}{}           & \multicolumn{1}{l}{}                 \\ \hline
CodeGen2                 & 7B                             & Instruct                        &                                  &                                & Yes                                  \\
Starcoder-15.5B          & 15.5B                          & Instruct                        &                                  &                                & Yes                                  \\
Vicuna                   & 7B                             & Instruct                        &                                  &                                & No                                   \\
nsql-6B                  & 6B                             & Seq2Seq                         &                                  &                                & Yes                                  \\ \hline
T5-3B(tscholak/cxmefzzi) & 3B                             & Seq2Seq                         &                                  &                                & Yes                                  \\
PICARD+T5/3B             & 3B                             & Seq2Seq                         &                                  &                                & Yes                                  \\ \hline
\end{tabular}
\end{table*}

==> tables_results/Models.tex <==



==> tables_results/SQAM.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\begin{tabular}{llr}
\hline
Model Type                         & Model Name               & \multicolumn{1}{l}{All} \\ \hline
\multirow{8}{*}{General LLM}       & ChatGPT-3.5-turbo        & 72.8                    \\
                                   & Davinci                  & 54.7                    \\
                                   & MPT-7B-instruct          & 55.7                    \\
                                   & ALPACA-7B                & 57.2                    \\
                                   & KOALA-7B                 & 44.4                    \\
                                   & OpenAssistant-pythia-12B & 49.1                    \\
                                   & Falcon-7B-instruct       & 38.9                    \\
                                   &                          & \multicolumn{1}{l}{}    \\ \hline
\multirow{4}{*}{Code Specific LLM} & CodeGen2-7B              & 61.5                    \\
                                   & Starcoder-15.5B          & 65.0                    \\
                                   & Vicuna-7B                & 42.9                    \\
                                   & nsql-6B                  & 81.4                    \\ \hline
\multirow{2}{*}{Seq-to-Seq Model}  & T5-3B(tscholak/cxmefzzi) & 84.3                    \\
                                   & PICARD+T5/3B             & 84.7                    \\ \hline
\end{tabular}
\end{table}
